Semi-Quantum Money

Quantum money allows a bank to mint quantum money states that can later be verified and cannot be forged. Usually, this requires a quantum communication infrastructure to transfer quantum states between the user and the bank. Gavinsky (CCC 2012) introduced the notion of classically verifiable quantum money, which allows verification through classical communication. In this work we introduce the notion of classical minting, and combine it with classical verification to introduce semi-quantum money. Semi-quantum money is the first type of quantum money to allow transactions with completely classical communication and an entirely classical bank. This work features constructions for both a public memory-dependent semi-quantum money scheme and a private memoryless semi-quantum money scheme. The public construction is based on the works of Zhandry and Coladangelo, and the private construction is based on the notion of Noisy Trapdoor Claw Free Functions (NTCF) introduced by Brakerski et al. (FOCS 2018). In terms of technique, our main contribution is a perfect parallel repetition theorem for NTCF.

==> macros.tex <==
\ifnum\sigconf=0\usepackage{authblk}
\fi 
\usepackage{silence} %authbulk must loaded before the silence package!!
\WarningFilter{latex}{BibTeX empty}
\WarningFilter{microtype}{`draft' option active}
\usepackage[modulo]{lineno}
\RequirePackage{etex}
\usepackage{amsthm,amssymb,amsfonts,latexsym,color,paralist,url,ifdraft,mathrsfs,thm-restate,comment,bbold,booktabs,subfig,array,tablefootnote,multirow}

\usepackage[utf8]{inputenc} \usepackage[autostyle=false, style=english]{csquotes} \MakeOuterQuote{"}
%csquotes after inputenc
\usepackage[T1]{fontenc}

\ifnum\sigconf=0
    \usepackage[draft=false,pageanchor,hyperindex,breaklinks]{hyperref}
    \usepackage[final]{graphicx}
\else
    \hypersetup{final}
\fi
%nomenclature related:
\usepackage[refpage,prefix]{nomencl}

\def\pagedeclaration#1{, \hyperlink{page.#1}{page\nobreakspace#1}}
\makenomenclature
\newcommand*{\nom}[3]{#1\nomenclature[#3]{#1}{#2}}
%end of nomenclature



%\usepackage[displaymath,textmath,sections,graphics,floats]{preview}
%\RequirePackage{silence}
\WarningFilter{l3regex}{This package is obsolete }
\WarningFilter{latex}{Float too large for page}

\usepackage [ lambda,advantage , operators , sets , adversary , landau , probability , notions , logic ,ff, mm,primitives , events , complexity , asymptotics , keys]{cryptocode}
%\usepackage{mathtools} \mathtoolsset{showonlyrefs}    %show only equations which are referenced laterside
%\usepackage[capitalise]{cleveref} %Incompatible with showonlyrefs

%the following commands are defined by crptocode. Define these ourselves if needed: \newcommand{\poly}{\mathrm{poly}} \newcommand{\prob}[1]{\Pr[ #1 ]} \newcommand{\norm}[1]{\left\| #1 \right\|} \newcommand{\RR}{\mathbb{R}} \newcommand{\FF}{\mathbb{F}} \newcommand{\CC}{\mathbb{C}} \newcommand{\NN}{\mathbb{N}}\DeclarePairedDelimiter\ceil{\lceil}{\rceil} \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\renewcommand{\verify}{\ensuremath{\mathsf{verify}}} 
\newcommand{\cverify}{\ensuremath{\mathsf{cverify}}}
\newcommand{\qverify}{\ensuremath{\mathsf{qverify}}}



%\renewcommand{\sfdefault}{phv}
%\renewcommand{\rmdefault}{ptm}
\theoremstyle{plain}
  
\ifnum\sigconf=0
    \newtheorem{theorem}{Theorem}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{definition}[theorem]{Definition}
    \newtheorem{example}[theorem]{Example}
    \newtheorem{conjecture}[theorem]{Conjecture}
\fi 
  \newtheorem{claim}[theorem]{Claim}
  \newtheorem{fact}[theorem]{Fact}
  \newtheorem*{theorem*}{Theorem}
  \newtheorem*{lemma*}{Lemma}
  \newtheorem*{corollary*}{Corollary}
  \newtheorem*{proposition*}{Proposition}
  \newtheorem*{claim*}{Claim}
  
  \theoremstyle{definition}
  \newtheorem{openproblem}[theorem]{Open Problem}
  \theoremstyle{remark}
  \newtheorem{remark}[theorem]{Remark}

  \theoremstyle{plain}
  \renewcommand{\qedsymbol}{$\square$}

% ---------------------------------------------------------------------------
\ifdraft{\newcommand{\authnote}[3]{{\color{#3} {\bf  #1:} #2}}}{\newcommand{\authnote}[3]{}}
\newcommand{\note}[1]{{\color{red}#1}}
%Example for how this should be used, in main file:
%\newcommand{\onote}[1]{\authnote{Or}{#1}{blue}}


\newcommand{\CNOT}{\mathrm{CNOT}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}

\newcommand{\const}{\mathrm{const}}

\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}
\newcommand{\ketbra}[1]{\vert #1 \rangle \langle #1 \vert}
\newcommand{\braket}[2]{\langle #1 \vert #2 \rangle}
\newcommand{\conjugate}[1]{#1^{\dagger}}
\newcommand{\tensor}{\otimes}
\DeclareMathOperator{\tr}{Tr}
\newcommand{\transpose}[1]{#1^{\mathsf{T}}}
\ifnum\sigconf=0
    \ifdraft{\usepackage{showlabels}}{} %must be after use package{hyperref}.
    \ifdraft{\linenumbers}{}
\fi

\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\E}{\mathbb{E}}

%\PreviewMacro*\onote
%\PreviewMacro*\nom
%\PreviewMacro*\ifdraft
%\DeclareMathOperator*{\E}{\scalerel*{\mathbb{E}}{\textstyle\sum}}


\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%document specific
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage[normalem]{ulem}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\sR}{\mathcal{R}}
\newcommand{\inj}{J}
\newcommand{\Es}[1]{\textsc{E}_{#1}}
\newcommand{\dset}{G}
\newcommand{\BQP}{\textsf{BQP}}
\renewcommand{\supp}{\textsc{Supp}}
\newcommand{\decrypt}{\ensuremath{\mathsf{decrypt}}}
\newcommand{\encrypt}{\ensuremath{\mathsf{encrypt}}}
\newcommand{\otr}{\ensuremath{\mathsf{OTR}}}
\newcommand{\ot}{\ensuremath{\mathsf{OT}}}
\newcommand{\ts}{\ensuremath{\mathsf{TS}}}
\newcommand{\ds}{\ensuremath{\mathsf{DS}}}
\newcommand{\tm}{\ensuremath{\mathsf{TM}}}
\newcommand{\stamp}{
 {\mathchoice
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.2ex]{RubberStamp}}
  {\includegraphics[height=0.9ex]{RubberStamp}}
 }
}
%\newcommand{\keygen}{\ensuremath{\mathsf{key\textit{-}gen}}}
\newcommand{\tokengen}{\ensuremath{\mathsf{token\textit{-}gen}}}
%\newcommand{\sign}{\ensuremath{\mathsf{sign}}}
%\newcommand{\verify}{\ensuremath{\mathsf{verify}}}
\renewcommand{\mac}{\ensuremath{\mathsf{mac}}}


\usepackage{tikz}
\usetikzlibrary{arrows,chains,matrix,positioning,scopes}
%
\makeatletter
\tikzset{join/.code=\tikzset{after node path={%
\ifx\tikzchainprevious\pgfutil@empty\else(\tikzchainprevious)%
edge[every join]#1(\tikzchaincurrent)\fi}}}
\makeatother
%
\tikzset{>=stealth',every on chain/.append style={join},
         every join/.style={->}}
\tikzstyle{labeled}=[execute at begin node=$\scriptstyle,
   execute at end node=$]
%

\ifnum\sigconf=0
    \usepackage[capitalise]{cleveref} %Incompatible with showonlyrefs
\fi
%\usepackage{autonum}%must be loaded after cleveref. Sometimes causes bugs. The alternative is incomaptible with cleveref:
 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases. In any case, showonlyrefs does not work with cleveref.



%Abstract:
%\newcommand{\ab}[1]{#1} \newcommand{\fv}[1]{}

%Full version:
\newcommand{\ab}[1]{} \newcommand{\fv}[1]{#1} %%


\ifnum\masterthesis=1
    \usepackage{setspace}
    \onehalfspacing
    \usepackage{fancyhdr}
    \pagestyle{fancy}
    \fancyhf{}
    \renewcommand{\headrulewidth}{0pt}
    \renewcommand{\headheight}{14pt}
    \chead{\thepage}
    
    \usepackage{pdfpages}
    
    \newcommand{\longunderline}{\underline{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }\ }
    
    \newenvironment{changemargin}[2]{%
        \begin{list}{}{%
        \setlength{\topsep}{0pt}%
        \setlength{\leftmargin}{#1}%
        \setlength{\rightmargin}{#2}%
        \setlength{\listparindent}{\parindent}%
        \setlength{\itemindent}{\parindent}%
        \setlength{\parsep}{\parskip}%
        }%
    \item[]}{\end{list}}
\fi


\newcommand{\forger}{\mathcal{F}}
\renewcommand{\dist}{\mathcal{D}}
\newcommand{\fulladv}{\mathcal{A}}
\newcommand{\miniadv}{\mathcal{B}}
\newcommand{\twominiadv}{\mathcal{C}}
\newcommand{\solver}{\mathcal{S}}
\newcommand{\solvertwo}{\mathcal{T}}
\newcommand{\boltforger}{\mathcal{L}}
\newcommand{\certforger}{\mathcal{C}}

\newcommand{\counterfeit}[3]{\ensuremath{\mathsf{COUNTERFEIT}}_{#1, #2}^{#3}(\secpar)}
\newcommand{\macforge}[1]{\ensuremath{\mathsf{MAC\text{-}FORGE}}_{\forger, #1}(\secpar)}
\newcommand{\solveboth}[1]{\ensuremath{\mathsf{SOLVE\text{-}2}}_{\solvertwo, #1}(\secpar)}
\newcommand{\solve}[1]{\ensuremath{\mathsf{SOLVE}}_{\solver, #1}(\secpar)}
\newcommand{\sigforge}[1]{\ensuremath{\mathsf{SIG\text{-}FORGE}}_{\forger, #1}(\secpar)}
\newcommand{\boltforge}[1]{\ensuremath{\mathsf{FORGE\text{-}BOLT}}_{\boltforger, #1}(\secpar)}
\newcommand{\certforge}[1]{\ensuremath{\mathsf{FORGE\text{-}CERTIFICATE}}_{\certforger, #1}(\secpar)}
\newcommand{\sabmoney}[2]{\ensuremath{\mathsf{SABOTAGE\text{-}MONEY}}_{#1, #2}(\secpar)}

\newcommand{\ql}{\ensuremath{\mathsf{QL}}}
\newcommand{\setup}{\ensuremath{\mathsf{setup}}}
\newcommand{\genbolt}{\ensuremath{\mathsf{gen\text{-}bolt}}}
\newcommand{\verbolt}{\ensuremath{\mathsf{verify\text{-}bolt}}}
\newcommand{\gencert}{\ensuremath{\mathsf{gen\text{-}certificate}}}
\newcommand{\vercert}{\ensuremath{\mathsf{verify\text{-}certificate}}}
\newcommand{\signscheme}{\ensuremath{\mathsf{DS}}}

\newcommand{\quantumcom}{\ensuremath{\Rightarrow}}
\newcommand{\doublequantumcom}{\ensuremath{\Leftrightarrow}}
\newcommand{\singleclassiccom}{\ensuremath{\rightarrow}}
\newcommand{\classiccom}{\ensuremath{\leftrightarrow}}
\newcommand{\payer}{\ensuremath{P}}
\newcommand{\receiver}{\ensuremath{R}}
\newcommand{\bank}{\ensuremath{B}}
\newcommand{\acquirer}{\ensuremath{A}}

\newcommand{\mybib}{\bibliography{semi_quantum_money}}

%\declaretheorem[name=Theorem,numberwithin=section]{thm}

\newcommand{\nextver}[1]{}

\newcommand{\figspace}{\ \ \ \ \ \ \ \ \ \ \ \ }
\newcommand{\minifigscale}{0.4}
\newcommand{\tablefigscale}{0.5}

\renewcommand{\sample}{\ensuremath{\gets}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% end macros

